Moshi Moshi? A Model Selection Hijacking Adversarial Attack

Model selection is a fundamental task in Machine Learning~(ML), focusing on selecting the most suitable model from a pool of candidates by evaluating their performance on specific metrics. This process ensures optimal performance, computational efficiency, and adaptability to diverse tasks and environments. Despite its critical role, its security from the perspective of adversarial ML remains unexplored. This risk is heightened in the Machine-Learning-as-a-Service model, where users delegate the training phase and the model selection process to third-party providers, supplying data and training strategies. Therefore, attacks on model selection could harm both the user and the provider, undermining model performance and driving up operational costs. In this work, we present MOSHI (MOdel Selection HIjacking adversarial attack), the first adversarial attack specifically targeting model selection. Our novel approach manipulates model selection data to favor the adversary, even without prior knowledge of the system. Utilizing a framework based on Variational Auto Encoders, we provide evidence that an attacker can induce inefficiencies in ML deployment. We test our attack on diverse computer vision and speech recognition benchmark tasks and different settings, obtaining an average attack success rate of 75.42%. In particular, our attack causes an average 88.30% decrease in generalization capabilities, an 83.33% increase in latency, and an increase of up to 105.85% in energy consumption. These results highlight the significant vulnerabilities in model selection processes and their potential impact on real-world applications.

==> sections/mshaa.tex <==
\section{Model Selection Hijacking Adversarial Attack}
In this section, we introduce the MSHAA, discussing the motivation behind the attack, the methodology employed, and the tools developed to poison the victim’s validation set. We provide a detailed overview of how MSHAA manipulates the model selection process by strategically injecting adversarial samples, ensuring that the attacker's desired model is favored.
\subsection{Motivations}
%\lpasa{se siete d'accordo io useri ML e non AI. di fatto l'AI non ha bisogno della model selection (e chiamre AI il ML è abbstanza sbagliato a mio parare)}
Model selection is a critical step in the ML 
%AI 
development process due to its profound impact on the performance, efficiency, and generalizability of the resulting system. The choice of model determines how well the 
%AI 
ML model can learn from data, adapt to new information, and perform tasks accurately. Selecting an appropriate model involves evaluating various algorithms and architectures to identify the one that best fits the specific problem domain and dataset characteristics. This process ensures that the ML system can achieve optimal performance while minimizing overfitting and underfitting, thereby enhancing its robustness and reliability in real-world applications.
\par
Although extremely critical, works on AML did not consider \textit{if} and \textit{how} the model selection can be tampered with by adversaries for some advantage.  
In this work, we aim to answer this research question by presenting the \textit{Model Selection Hijacking Adversarial Attack} (MSHAA), a novel adversarial vector to ML applications. 
%
\subsection{Adversary Goal}
The goal of our proposed attack -- the \textit{Model Selection Hijacking Adversarial Attack} (MSHAA) -- is to control the model selection phase by injecting malicious crafted samples to the solely validation set.  
In this scope, the adversary goal is to let the model selection phase select the model architecture that suit the best a target metric, named \textit{hijack metric} $m$. 
The hijack metric is arbitrary and can be chosen by the adversary. 
%Last, we assume adversaries cannot alter the standard model selection routine, meaning they cannot alter the loss metric defined by the victim, nor the underling code.This means that with MSHAA we inject samples that alter the validation loss in such a way that the model that fits the best the hijack metric also result with a lower loss compared to the other models in the grid. 
Lastly, we assume that adversaries cannot modify the standard model selection routine, including the loss metric defined by the victim, the underlying code, or the model selection policy. This means that with MSHAA, we inject samples that influence the loss function evaluation on the validation set, ensuring that the model best suited to the hijack metric also achieves a lower loss compared to other models in the validation grid.
In this work, we explore different types of hijack metrics. 

%
\subsubsection{Threat Model}
Suppose the victim has access to a dataset $\mathcal{S}$, divided in train $\mathcal{S}^{Train}$, validation $\mathcal{S}^{Val}$, and testing $\mathcal{S}^{Test}$ sets.%\lpasa{occhio che sta divisione senza Resampling non è affrontata nel cap Background attualmente}
%
The former is used to train several model $h_{\mathfrak{c}}$ grouped in a models %grid 
set identifiable with $\mathfrak{C}$,\footnote{$\mathfrak{c}$ represents the configuration of hyperparameters and $\mathfrak{C}$ the set of all possible configurations of hyperparameters.} the second to perform model selection, and the latter to test the best model performance. %generalization capability.
%The model selection phase will then return the best model $h_{\mathfrak{c}^*}$, which is defined as the model, among the ones trained, that has the lowest validation loss: 
The model selection phase will return the model $h_{\mathfrak{c}^*}$ with the lowest true error estimate on the validation set among those trained:
    \begin{equation}
        \label{best_val}
 h_{\mathfrak{c}^*} = \argmin_{h_{\mathfrak{c}} : \mathfrak{c} \in \mathfrak{C}} \mathcal{L}_{Val}(h_{\mathfrak{c}}, \mathcal{S}^{Val}).
    \end{equation}

In this context, we postulate that the adversary possesses access to the validation set $\mathcal{S}^{Val}$, enabling them to read and modify its data. Consequently, our newly proposed adversarial family, MSHAA, exhibits characteristics akin to data poisoning, as it allows the attacker to alter the victim’s dataset.
In contrast with the traditional poisoning attack, our proposed MSHAA operates solely at the validation set level, leaving the training set unaltered. 
\par
We now outline the adversary knowledge, detailing the information and capabilities that an attacker possesses, as well as the limitations and constraints they face within our threat model.
We explore two distinct attack settings.
\begin{itemize}
    \item \textit{White-box attack}: adversaries with full knowledge of the  trained models $h_{\mathfrak{c}}, \;  \forall c \in \mathcal{C}$ (\textit{i.e., architectures, trained parameters} and they can freely query the model for inference purposes).  
    \item \textit{Black-box attack}: adversaries with knowledge limited to the model's architectures $\mathfrak{C}$ (\textit{i.e.,} the models that will be learned and tested during the model selection phase). 
\end{itemize}
Furthermore, in both scenarios adversaries know $\mathcal{S}^{Train}$ but they cannot tamper it. 
We again recall that -- for both white-box and black box settings -- the attacker is limited to modifying of the only validation set $\mathcal{S}^{Val}$.
A schematic representation of the considered threat model is depicted in Figure~\ref{fig:overview}.

\begin{figure*}[!htpb]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/attack_overview.pdf}
    \caption{Schematic representation of the MSHAA threat model.}
    \label{fig:overview}
\end{figure*}


\subsubsection{Stealthiness}
Poisoning only the validation set allows all the trained models and their parameters not to be modified during the attack. This means that once attacked, the model selection phase, which is carried out in an unmodified way, returns a model that has been regularly trained on clean data, and among all the ones trained is of higher hijack metric, which can be chosen by the adversary. 
%This means that the returned model does not leak any clue about the attack having been carried out, but on the other hand, limits the effectiveness of the attack itself based on the hijack metric of the available models.
This ensures that the selected model reveals no evidence of the attack, as its performance on the victim's loss function remains close to that of models selected using the original validation data. However, it differs in terms of the hijack metric, which is influenced to align with the attacker’s desired outcome.

\subsubsection{Threat Victims}
With MSHAA attack execution might impact different victims through traditional poisoning and backdoor dynamics~\cite{tian2022comprehensive, li2022backdoor}. 
A pertinent example within the context of a threat model is the public dissemination of datasets, which are typically pre-structured into standard partitions (training, validation, and testing splits) to facilitate the reproducibility of experimental outcomes. In such a scenario, tampering with the validation set represents a significant vulnerability, as it undermines the integrity and reliability of the results. 
The attacker provides a compromised dataset to a service provider, to increase the inefficiency of its services by increasing, for instance, the energy consumption or the latency in the predictions, or, conversely, aiming to produce a stealthy poisoning attack by altering the victim's model performance. 
% Furthermore, in the context of the MLaaS paradigm, the attack can be three-fold:

% \begin{itemize}
%     \item The attacker provides a compromised dataset to a service provider, to increase the inefficiency of its services by increasing, for instance, the energy consumption or the latency in the predictions. 
%     \item The victim provides the dataset and a training strategy to the MLaaS provider, whose goal is to train a model with powerful hardware and returned the optimal model to the victim. Here, the MLaaS provider might tamper the 
% \end{itemize}


==> sections/results.tex <==
% \section{Results -- OLD}
% MSHAA was tested against sets of models grouped into model grids \textcolor{blue}{set} based on some hyperparameters (e.g. the number of neurons per layer in the MNIST case study) and/or based on the learning rate used for training.\lpasa{il concetto di model grid va un po spiegato, nel senso che noi non parliamo mai di grid search al momento, e quindi non si capisce perche si definisca come griglia e non come set (per come è adesso secondo me è più corretto usare set))} 

% \subsection{Evaluation Metrics}
% In order to qualitatively estimate the effectiveness of the
% attack against the specific model’s grid set considered, we
% introduce two distinct metrics: the \textit{Effectiveness Score Function} (ESF) and the \textit{Attack Success Rate} (ASR).
    
% \paragraph{Effectiveness Score Function}
% % In order to qualitatively estimate the effectiveness of the attack against the specific \textcolor{red}{model's grids} \textcolor{blue}{set} considered, we introduce the \textit{Effectiveness Score Function} (ESF). 
% The ESF goal is to understand the impact of MSHAA on the victim model when deployed. Therefore, with ESF we measure the MSHAA returned model $\tilde{h}_{\mathfrak{c}^*}$ and the legitimate $h_{\mathfrak{c}^*}$ based on the hijack metric $\mathcal{E}$.
% Formally, ESF is defined as follows:
% \begin{equation}
%      \mathscr{S}(\mathfrak{C}) = \frac{
%          \mathcal{E} ( \tilde{h}_{\mathfrak{c}^*}, \mathcal{S}^{Test} ) 
%          - 
%          \mathcal{E} ( h_{\mathfrak{c}^*}, \mathcal{S}^{Test} )
%      }
%      {
%          \underset{\mathfrak{c} \in \mathfrak{C}}{\max} \{\mathcal{E}(h_{\mathfrak{c}}, \mathcal{S}^{Test})\} - 
%          \mathcal{E} (    h_{\mathfrak{c}^*}, \mathcal{S}^{Test}    )
%      }.
% \end{equation}

% ESF takes the difference between a chosen metric $\mathcal{E}$ of the models $\tilde{h}_{\mathfrak{c}^*}$ (see Eq.~\ref{best_poison}) and $h_{\mathfrak{c}^*}$ (see Eq.~\ref{best_val}) normalizing it with the difference between the maximum possible chosen metric of a model $h_\mathfrak{c}$ with $\mathfrak{c} \in \mathfrak{C}$, and again the chosen metric by $h_{\mathfrak{c}^*}$.\\
% This function allows us to evaluate our attack with any metric $\mathcal{E}$, for the purpose of this study, with regards to the hijack metric considered:
% \begin{itemize}
%     \item \texttt{Generalization Metric}. $\mathcal{E}$ is the loss function computed on the original validation set;
%     \item \texttt{Latency Metric}. $\mathcal{E}$ is the latency while processing the test set.
%     \item \texttt{Energy Consumption} or \texttt{$\ell_0$ Norm}. $\mathcal{E}$ is the estimated energy consumed by the model while processing the test set. When testing the attack in the SpeechCommands case, as we could not compute the \texttt{Energy} metric, we evaluated the quality of the attack using the \texttt{$\ell_0$ Norm}, by adopting $\mathcal{E}$ to be the $\ell_0$ Norm.
% \end{itemize}
% This Effectiveness Score function allows us to give a normalized score that sums up the effectiveness of the MSHAA, as a matter of fact:
% \begin{itemize}
%     \item \textit{Successful}, when $ESF > 0$, the MS phase to return a model with higher $\mathcal{E}$ compared to $h_{\mathfrak{c}^*}$. If the score is equal to $1.0$, then the returned model $\tilde{h}_{\mathfrak{c}^*}$ is the one among the considered models to have the highest $\mathcal{E}$.
%     \item \textit{Invariant}, when $ESF = 0.0$, the attack did not sway the MS phase, and the returned model is $\tilde{h}_{\mathfrak{c}^*} = h_{\mathfrak{c}^*}$, \textit{i.e.} the returned model is also the legitimate one. 
%     \item \textit{Unsuccessful}, $ESF < 0.0$ imply that the attack made the MS phase return a model of less $\mathcal{E}$ compared to $h_{\mathfrak{c}^*}$.
% \end{itemize}  

% \paragraph{Attack Success Rate}
% We define the ASR as a simplification of the ESF. In particular, we define the ASR as a boolean variable of a successful or unsuccessful attack, and therefore the $ASR = 1$ if $ESF > 0$, $ASR = 0$ otherwise. 
% With this metric, we are interested in understanding when an attack is successful in terms of increasing the hijack metric. 

% \subsection{Victim \textcolor{red}{Model's Grids}}
% Regardless of the case study at hand, we conduct conducted the attacks by considering each task's whole model's grids but also subsets. 
% For instance, in the MNIST case, we execute the attack when considering the whole grid (\textit{i.e.} the number of layers, number of neurons, learning rate) but also cases where we fixed - for instance - the learning rate and we vary the other two hyper parameters. 
% With this experimental setting, we aim to understand the attack effectiveness at different granularity. 
% Regardless of the case study at hand, we considered the victim models grouped in model grids based on some hyperparameters and/or based on the learning rate used for training. 
% In more detail, the chosen hyperparameter is:
% \begin{itemize}
% 	\item \textbf{MNIST Case}. Number of neurons per layer. Therefore, we obtain 18 sets of 10 models when grouping by learning rate and neurons, and 6 sets of 30 when grouping just by learning rate.
% 	\item \textbf{CIFAR10 Case}. Number of neurons in the second-to-last fully connected layer. Obtaining 6 sets of 7 models grouping by learning rate and neurons, and 2 sets of 21 models when grouping by learning rate.
% 	\item \textbf{SpeechCommands Case}. Number of neurons in the second-to-last fully connected layer. Having 4 sets of 4 models if we group by learning rate and neurons, and 2 sets of 8 models when grouping by just learning rate.
% \end{itemize}

% \subsection{Attacker Knowledge}
% In both white box and black box settings, we assume that the attacker has some different amount of knowledge at his disposal when launching the attack. In other words, we used sets of the models either clean or surrogate (obtained the same way as the aforementioned model grids), to train the HVAE.\\
% All in all, for the case studies at hand, we trained:
% \begin{itemize}
% 	\item \textbf{MNIST Case}. For each of the 6 considered learning rates, we assumed as knowledge possessed by the attacker, the 10 models having 32, 64, or 128 neurons separately and together, amounting to 24 overall HVAE trained (4 HVAE for each learning rate).
% 	\item \textbf{CIFAR10 Case}. For each of the 2 considered learning rates, we assumed as knowledge possessed by the attacker, the 7 models having the second to last fully connected layer with 128, 256, or 512 neurons, taken singularly or together, for a total of 8 HVAE trained.
% 	\item \textbf{SpeechCommands Case}. For each of the 2 considered learning rates, we assumed as knowledge possessed by the attacker, the 4 models having the second to last fully connected layer with 128, 256 neurons, taken singularly or together, for a total of 6 HVAE trained.
% \end{itemize}

\section{Results}
We analyze the impact of the MSHAA attack on the experimental settings previously described.
As MSHAA generates malicious poisoning samples to inject into the validation set, we explore the attack effect in two fashions:
\begin{itemize}
    \item \textit{Full substitution}, where the validation set is entirely substituted by the malicious samples. 
    \item \textit{Partial substitution}, where the validation set combines both legitimate and malicious samples at different rates (\textit{i.e.} 10\%, 20\%, 50\%, 80\%, 100\%). 
\end{itemize}
We measure the attack performance by comparing -- for each grid attack presented in Table~\ref{tab.grid} -- the legitimate model (\textit{i.e.} the model with the lowest loss in the unpoisoned validation set) and the malicious model (\textit{i.e.} the model with the lowest loss in the poisoned validation set). 

\subsection{Full Substitution}
Tables~\ref{tab.asr-wb} and \ref{tab.asr-bb} show the results of MSHAA in both white-box and black-box, respectively. Each table is composed by three sub-tables that represent the three distinct attack grid granularities,  \textit{i.e.} global, grouped-by learning rate, and grouped-by learning rate and number of neurons. For each case, we report the results for the three case studies (\textit{i.e.} MNIST, CIFAR10, and Speech Commands) spanning across the four studied hijack metrics (\textit{i.e} generalization error, latency, energy, and $\ell_0$. 
Furthermore, each row reports the number of sets. \footnote{Each set we trained an ad-hoc HVAE (see Sec.~\ref{ssec.grid}).} Consider Table~\ref{tab.asr-bb} on the MNIST use-case and global granularity: since we have only 1 set, the attack is either successful (100\%) or unsuccessful (0\%).
\par
Overall, we denote strong positive results proving the validity of HVAE, this first approach we proposed to address an MSHAA. 
The attack is perfectly successful (\textit{i.e.} $ASR = 100\%$) in $22/33$ and $23/33$ cases in both white-box and black-box scenarios.
Interestingly, we do not observe differences between white and black box settings, implying that the attack can be very dangerous, yielding high transferability capabilities. 
\par
The proposed attack appears to be extremely dangerous, especially for the generalization: in all the considered cases, our HVAE produced a poisoned validation set that hijacked the model selection, always returning a non-optimal that generalizes less. 
\par
Last, while our proposed attack HVAE shows promising results across different benchmarks, it suffers from the increased complexity of the data. In particular, in the SpeechCommands, the attack fails to produce poisoned validation samples capable of hijacking the model selection.   
%This phenomenon might be due to HVAE's underlying architecture which is not optimal in learning useful representation. 
This phenomenon may be attributed to the underlying architecture of the HVAE, which is not well-suited for learning effective representations in sequential domains.
We believe that future studies might attempt to design ad hoc HVAE for specific tasks (e.g., RAVE for the Speech domain~\cite{caillon2021rave}).
\par
We can therefore conclude that our proposed attack HVAE is effective and can produce strong manipulations to the model selection phase. Furthermore, these results answer our original research question: \textit{can an attacker manipulate the model selection?} The answer is yes, we can produce an MSHAA attack, and an attacker can ideally choose custom hijack metrics.  

\begin{table}[!htpb]
\centering
\footnotesize
\caption{ASR in White-Box Settings at different attack grid granularities.}
\begin{tabular}{c|c|c|c|c|c}  \toprule
\multicolumn{6}{c}{\textit{\textbf{Global}}} \\ \midrule
 & \textit{\# Sets} &\textit{Gener.} & \textit{Latency} & \textit{Energy} & \textit{$\ell_0$} \\ \midrule
MNIST & 1 & 100.0\% & 100.0\% & 100.0\% & 100.0\% \\
CIFAR10 & 1 &100.0\% & 0.0\% & 100.0\% & 100.0\% \\
SpeechC. & 1 & 100.0\% & 0.0\% & N/A & 0.0\% \\ \midrule
\multicolumn{6}{c}{\textit{\textbf{Learning Rate}}} \\ \midrule
MNIST & 6 &  100.0\% & 100.0\% & 66.7\% & 83.3\% \\
CIFAR10 & 2 & 100.0\% & 100.0\% & 100.0\% & 100.0\% \\
SpeechC. & 2 & 100.0\% & 50.0\% & N/A & 0.0\% \\\midrule
\multicolumn{6}{c}{\textit{\textbf{Learning Rate \& \# Neurons}}} \\ \midrule
MNIST & 18 & 100.0\% & 94.4\% & 100.0\% & 100.0\% \\
CIFAR10 & 6 & 100.0\% & 33.3\% & 50.0\% & 50.0\% \\
SpeechC. & 4 & 100.0\% & 50.0\% & N/A & 0.0\% \\ \bottomrule
\end{tabular}
\label{tab.asr-wb}
\end{table}

\begin{table}[!htpb]
\centering
\footnotesize
\caption{ASR in Black-Box Settings at different attack grid granularities.}
\begin{tabular}{c|c|c|c|c|c}  \toprule
\multicolumn{6}{c}{\textit{\textbf{Global}}} \\ \midrule
 & \textit{\# Sets} & \textit{Gener.} & \textit{Latency} & \textit{Energy} & \textit{$\ell_0$} \\ \midrule
MNIST & 1 & 100.0\% & 100.0\% & 100.0\% & 100.0\% \\
CIFAR10 & 1   & 100.0\% & 100.0\% & 100.0\% & 100.0\% \\
SpeechC.  & 1 & 100.0\% & 0.0\% & N/A & 0.0\% \\ \midrule
\multicolumn{6}{c}{\textit{\textbf{Learning Rate}}} \\ \midrule
MNIST & 6 &  100.0\% & 100.0\% & 66.7\% & 83.3\% \\
CIFAR10 & 2 & 100.0\% & 50.0\% & 50.0\% & 100.0\% \\
SpeechC. & 2 & 100.0\% & 50.0\% & N/A & 0.0\% \\ \midrule
\multicolumn{6}{c}{\textit{\textbf{Learning Rate \& \# Neurons}}} \\ \midrule
MNIST & 18 & 100.0\% & 83.3\% & 100.0\% & 100.0\% \\
CIFAR10 & 6 & 83.3\% & 50.0\% & 33.3\% & 50.0\% \\
SpeechC. & 4 & 100.0\% & 50.0\% & N/A & 50.0\% \\ \bottomrule
\end{tabular}
\label{tab.asr-bb}
\end{table}

\subsection{Partial Substitution}
We now analyze the impact on the validation poisoning rate. 
Figures~\ref{fig:pr-impact-lr} and~\ref{fig:pr-impact} show such a trend on the grid attack settings \textit{learning rate} and \textit{learning rate \& \#neurons}, respectively, where we report the three use cases, the four hijack metrics, and both knowledge levels. 
By analyzing the ESF for the first two datasets considered, we can observe that the white-box settings are useful to produce a stronger attack, which is comparable to more traditional poisoning properties. Despite that, we do not observe clear advantages in poisoning the validation set entirely. This result suggests that HVAE can produce an effective attack even by tampering with only a smaller portion of the validation set.\\
On the other hand, in the Speech Commands case study, we observe a more erratic behavior of the mean ESF. This is particularly evident for the $\ell_0$ hijack metric, despite achieving an Attack Success Rate greater than zero, as illustrated in Figures ~\ref{fig:pr-impact-lr} and~\ref{fig:pr-impact}, the mean ESF of these attacks is heavily below 0,  This discrepancy arises because, for some attacks, the ESF values are strongly negative.
We believe that in future works the interplay between MSHAA effectiveness and the poisoning rate should be explored. 

\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/pr_impact_lr.pdf}
    \caption{Poisoning rate impact on the grid attack setting ``\textit{learning rate}'' for both White-Box (WB) and Black-Box (BB) knowledge level. }
    \label{fig:pr-impact-lr}
\end{figure}
 
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/pr_impact.pdf}
    \caption{Poisoning rate impact on the grid attack setting ``\textit{learning rate \& \#neurons}'' for both White-Box (WB) and Black-Box (BB) knowledge level. }
    \label{fig:pr-impact}
\end{figure}


\subsection{Impact on the Availability}
%\textbf{INTRO per Riccardo. Ricorda di dire che i risultati soon in 100\% val poisoned. Analizza brevemente anche see vedi difference tra white and black box settings.} 
In this section, we present the impact of our attack on the targeted metrics for the specific case study and models considered. 
In Table \ref{tab.impact} we illustrate how MSHAA, by influencing the Model Selection phase, impacts the chosen metrics. This is done by reporting the ratio between the metrics of the model returned by an untampered Model Selection, and the model returned once the attack, conducted by training the HVAE with full knowledge of the victim models, and with full (100\%) substitution of the original validation set with poison data. 
For instance, when considering the white-box knowledge, we observed a malicious MNIST model $\times3$ slower that the legitimate model in terms of latency introduced. 
\par
As we can see from the table, the WB and BB settings perform similarly in both the MNIST and SpeechCommands case studies. The former presents the same model for all the attacks conducted with the various hijack metrics, and the latter shows better performance only for the WB case on the Generalization Metric. Finally, for the CIFAR10 case study, the BB setting performs slightly better, allowing for a small increase in the Latency metric.

\begin{table}[!htpb]
\centering
\footnotesize
\caption{Impact factor on the availability. The results report the impact factor. We only report the values for the \textit{global} attacker grid variant. }
\begin{tabular}{c|c|c|c|c}  \toprule
\multicolumn{5}{c}{\textit{\textbf{White-Box}}} \\ \midrule
 &\textit{Gener.} & \textit{Latency} & \textit{Energy} & \textit{$\ell_0$} \\ \midrule
MNIST  & 21.27 & 3.818 & 1.244 & 6.293 \\
CIFAR10 & 1.120 & 0.769 & 1.009 & 1.027 \\
SpeechC. & 4.136 & 0.797 & N/A & 0.629 \\ \midrule
\multicolumn{5}{c}{\textit{\textbf{Black-box}}} \\ \midrule
MNIST  & 21.27 & 3.818 & 1.244 & 6.293 \\
CIFAR10 & 1.180 & 1.001 & 1.009 & 1.027 \\
SpeechC. & 2.319 & 0.797 & N/A & 0.810 \\ \bottomrule
\end{tabular}
\label{tab.impact}
\end{table}

The study of the impact on the availability of our attacks reconfirms the strong link between our attack and the models for which is performed the model selection, as having a more bigger and diverse set of models allows us to have possibly higher metrics, which allows us to train more effective HVAE and a more impactful attack.

% \subsection{Results -- OLD}
% In order to evaluate the effectiveness of the MSHAA, we tested the attacks stemming from the trained HVAE, by substituting an increasing amount of the clean validation set with generated poisoning data (from substituting 10\% to substituting the whole clean validation set). We then computed the poisoned validation loss on the victim models that share the learning rate with the known models by the adversary.\\
% To evaluate the performance of the attack we divided the trained models into multiple sets, to assert if the attack was successful in swaying the Model Selection phase, by comparing the model with the lowest clean validation loss and the one with the lowest poison validation loss.\\
% To better present the performance of the attack, here we report the percentages of attacks able to achieve an effectiveness score greater than zero with regards to all the launched attacks. The reported percentages refer to attacks conducted substituting completely the validation set with poisonous samples.\\
% By way of example, in Tables \ref{WB-lr-n} and \ref{BB-lr-n}, we are considering the model set obtained by grouping per learning rate and number of neurons, therefore, for the MNIST case, we are testing the 4 HVAEs against the 18 model set for a total of 72 tests. Meanwhile, in Tables \ref{WB-lr} and \ref{BB-lr}, as we are working with the model set obtained by grouping just by the learning rate, in the MNIST case we are testing the 4 attacks against sets, amounting to 24 tests overall.

% \begin{table}[h!] \label{WB-lr-n}
%     \centering
%     \input{tables/attack_evaluation_WB_lr_neuron}
%     \caption{White box results lr \& neurons.}
% \end{table}

% \begin{table}[h!]\label{BB-lr-n}
%     \centering
%     \input{tables/attack_evaluation_BB_lr_neuron}
%     \caption{Black box results lr \& neurons.}
% \end{table}


% \begin{table}[h!]\label{WB-lr}
%     \centering
%     \input{tables/attack_evaluation_WB_lr}
%     \caption{Whitebox results lr.}
% \end{table}

% \begin{table}[h!]\label{BB-lr}
%     \centering
%     \input{tables/attack_evaluation_BB_lr}
%     \caption{Black box results lr.}
% \end{table}


% \subsection{Impact}



% %\textbf{Add some statistics on how the model results in terms of latency, energy, etc. Therefore, you compare based on each metric the value for the legitimate model, the hijacked one, and see how it increases. Therefore, I expect to see an average that says "it's 2.5 times slower than the legitimate model". The results should be represented as in the previous sec, therefore one paragraph for the overall grid, and then 4 distinct tables}
% Finally, we tested an attack with full knowledge of all the models in either the White Box or the Black Box setting, (i.e. for the MNIST case we assume the adversary knows all the trained 180 models). We then tested on sets containing all of the models, regardless of the learning rate used for training and the specific hyper-parameters considered. Following such an attack, we were able to succeed for both in White Box and Black Box Settings, in all tested metrics for the MNIST case. Meanwhile, for the CIFAR10 case, we did fail just on the \texttt{Latency} metric in the white box set. Finally, for the Speech Commands, we were able to succeed only with the \texttt{Generalization} metric.\\
% Now, by way of example, we report the impact of this last attack in the MNIST case, with respect to all of the considered hijack metrics, from all of the 180 trained models, the one that would be normally selected is composed of one layer of 128 neurons, trained at a learning rate of 0.001, having:
% \begin{itemize}
%     \item Clean Validation Loss:  0.000424  
%     \item Latency (s): 0.032640 
%     \item Estimated Energy Consumption (pJ): 2.289672e+07 
%     \item $\ell_0$ Norm: 79.473261 
% \end{itemize}

% Now, for this specific attack, when substituting the whole dataset with poisonous samples generated by our HVAE, for the specific metric considered, we have:
% \begin{itemize}
%     \item \texttt{Generalization Metric}. Launching the attack with this metric, we sway the MS phase into returning a model of 10 layers of 128 neurons trained at a learning rate of 0.005, that had a clean validation loss of 0.009013, spelling an increase of this metric of over 21.257 times.
%     \item \texttt{Latency Metric}. The model returned following this attack is the same as the Generalization metric, and has a latency of 0.124606 s, corresponding to an increase of 3.817 times.
%     \item \texttt{Energy Consumption}. With this metric, the MS returned the same model as before, which brings an estimated energy consumption of 2.848310e+07 pJ, representing an increase of 1.244 compared to the legitimately returned one.
%     \item \texttt{$\ell_0$ Norm}. This metric, again forced the MS to return the same model as before, and in terms of $\ell_0$ norm, we have 500.154926, which signifies an increase of 6.293.
% \end{itemize}


==> sections/settings.tex <==
\section{Experimental Settings}
We now describe the experimental settings utilized to demonstrate MSHAA attack. 
The experiments are conducted utilizing Python 3.10 scripts, and standard ML libraries to design deep learning experiments such as PyTorch~\cite{paszke2019pytorch}. 
All experiments are executed on a machine with 32GB RAM with an NVIDIA GeForce RTX 3090.
We publicly released our GitHub repository to reproduce our experiments fully: 
\url{https://anonymous.4open.science/r/MSHAA-68DD/README.md}

\subsection{Case Studies}
We designed three distinct case studies to test the MSHAA attack performance: two yield from the Computer Vision (CV) field, and the remaining one from Speech Recognition (SR), all in the classification task.
We opted to test these two distinct application domains %(CV and SR) 
to understand the generalization of the attack in different AI scenarios. 
We now briefly describe the three tasks.\footnote{All these datasets were imported using the corresponding PyTorch libraries.} 
\begin{itemize}
    \item \textit{MNIST (CV)~\cite{lecun2010mnist}}. It is a dataset of bilevel $28 \times 28$ handwritten digits divided into 10 classes: one for each digit from 0 to 9. The victim models considered for this case are FeedForward Neural Networks, with hyperparameters grid concerning the number of neurons per layer and the number of layers themselves. 
    \item \textit{CIFAR10 (CV)~\cite{cifar10}}. It is a dataset of colored $32 \times 32$ images of various subjects belonging to 10 classes: airplane, automobile, bird, cat, deer, dog, frog, horse, ship, and truck. In this case study the victim models are DenseNets \cite{huang2017densely}, of which we adapted the implementation done by \cite{PyTorchDenseNet}. The considered hyperparameters grid sees the number of dense blocks and the number of neurons for the fully connected layer which feeds the output one.
    \item \textit{Speech Commands (SR)~\cite{speechcommandsdataset}}. It is a dataset composed of audio files that are about 1 second long (around 16000 frames long) and belong to 35 classes of different commands spoken by different people. Here, the victim models are Convolutional Neural Networks composed of 1D convolutional layers, and the considered hyperparameters are the number of convolutional layers and the width of the fully connected layer that feeds the output one (code adapted from \cite{PyTorchSpeechCommands}).
\end{itemize}
All the models considered are feedforward neural networks, with an output composed of one or more dense layers that map the hidden representations to the output space. The architecture of the hidden layers varies depending on the specific task. A detailed list of the layers used is provided in Table \ref{tab.hp}.
In total, we trained 472 models, considering both white-box and black-box scenarios, 360 for MNIST, 84 for CIFAR10, and 32 for Speech Commands. 
Figure~\ref{fig:clean_samples} shows two examples for each dataset. Note that for the Speech Commands, we display the frequency spectrum. 

\begin{table}[!htpb]
\centering
\footnotesize
\caption{Hyper parameters grouped by use case. }
\begin{tabular}{cc} \toprule
\multicolumn{2}{c}{\textit{\textbf{MNIST}}} \\ \midrule
    $\#$ layers &     $[1, 2, 3, 4, 5, 6, 7, 8, 9, 10]$        \\
    $\#$ neurons &     $[32, 64, 128]$        \\
    $\#$ learning rate &     $[0.0001, 0.0005, 0.001, 0.005, 0.01, 0.05]$       \\ \midrule
    \multicolumn{2}{c}{\textit{\textbf{CIFAR10}}} \\ \midrule
    $\#$ dense blocks &     $[2, 3, 4, 5, 6, 7, 8]$        \\
    $\#$ neurons dense layer&     $[128, 256, 512]$        \\
    $\#$ learning rate &     $[0.001, 0.005]$       \\ \midrule
    \multicolumn{2}{c}{\textit{\textbf{Speech Commands}}} \\ \midrule
    $\#$ 1D conv layers &     $[2, 4, 6, 8]$        \\
    $\#$ neurons dense layer &     $[128, 256]$        \\
    $\#$ learning rate &     $[0.001, 0.005]$       \\ \bottomrule
\end{tabular}
\label{tab.hp}
\end{table}

\begin{figure}[!htpb]
    \centering
    \includesvg[width=0.5\linewidth]{figures/clean_samples}
    \caption{Illustration of samples from $\mathcal{S}^{Val}_{pois}$ for the three tasks: MNIST, CIFAR10, and Speech Commands.}
    \label{fig:clean_samples}
\end{figure}
 

\subsection{HVAE Implementations \& Attack Grid}\label{ssec.grid}
Regardless of the case study at hand, we conduct the attacks by considering each task's whole model's grids but also subsets. 
For instance, in the MNIST case, we execute the attack when considering the whole hyperparameters grid (\textit{i.e.} the number of layers, number of neurons, learning rate) but also cases where we fixed - for instance - the learning rate and we vary the other two hyper parameters. 
With this experimental setting, we aim to understand the attack effectiveness at different granularity. Table~\ref{tab.grid} describes the attack grid. 
For instance, when considering the MNIST scenario, we can execute the attack on the entire combination of hyperparameters (\textit{i.e.} learning rate, number of layers and neurons), consisting in one set containing 180 models, or, when grouping on the learning rate, we obtain 6 distinct sets (one per learning rate) constituted by 30 models ($3$ types of neurons $\times$ $10$ types of number of layers). 

\begin{table}[!htpb]
\centering
\footnotesize
\caption{Attack grid grouped by use case. }
\begin{tabular}{ccc} \toprule
\multicolumn{3}{c}{\textit{\textbf{MNIST}}} \\ \midrule
    \textit{Grouped-by} & \textit{\# sets} & \textit{\# models}\\ \hline
    Global &     1    &  180 \\
    learning rate &     6  &  30   \\
    learning rate \& $\#$ neurons &  18 &  10\\ \midrule
    \multicolumn{3}{c}{\textit{\textbf{CIFAR10}}} \\ \midrule
    Global &  1  &  42 \\
    learning rate &  2   & 21\\
    learning rate \& $\#$ neurons &    6    &   7 \\ \midrule
    \multicolumn{3}{c}{\textit{\textbf{Speech Commands}}} \\ \midrule
    Global &     1   &  16\\
    learning rate &   2  &  8 \\ 
    learning rate \& $\#$ neurons &    4   &  4  \\ \bottomrule
\end{tabular}
\label{tab.grid}
\end{table}
\par
In both white box and black box settings, we assume that the attacker has some different amount of knowledge at his disposal when launching the attack. In other words, we used sets of the models either clean or surrogate (obtained the same way as the aforementioned attack grid), to train the HVAE. In total, we trained 50 HVAE in MNIST: 25 sets over the three grouping conditions multiplied by the two knowledge levels (\textit{i.e.} white-box and black-box).
Similarly, we trained 18 and 14 HVAE for CIFAR10 and Speech Commands, respectively. 
\par
Finally, for each dataset, we trained HVAE with different architectures: 
\begin{itemize}
    \item \textit{MNIST}. The HVAE comprises only fully connected layers and is trained using Binary Cross Entropy as a reconstruction loss ($\mathcal{L}_{\mathrm{rec}}$). 
    \item \textit{CIFAR10}. For CIFAR10, the HVAE adopted is composed of 2D convolutional layers, and the adopted reconstruction loss ($\mathcal{L}_{\mathrm{rec}}$) is the Mean Square Error.
    \item \textit{Speech Commands}. The HVAE are made of 1D convolutional layers, with the Mean Square Error as the reconstruction loss ($\mathcal{L}_{\mathrm{rec}}$).
\end{itemize}

\subsection{Hijack Metrics}
We now describe the implementation details of the hijack metrics described in Section~\ref{ssec.hm-theory}. \textit{Generalization Metric}. This hijack metric consists of the loss obtained by our models when processing the original (legitimate) validation set. 
\textit{Latency Metric}: It is obtained by measuring the overall processing time of a given set of input data.
\textit{Energy Consumption}: it is computed by an ASIC simulator \footnote{\url{https://github.com/iliaishacked/sponge_examples}} \footnote{\url{https://github.com/Cinofix/sponge_poisoning_energy_latency_attack}} adapting the functions already developed for \cite{shumailov2021sponge} and \cite{cina2022energy}. As this tool was not compatible with the specific architecture used for the classification models of the SpeechCommands dataset, this was the only case in which we did not consider this specific metric.
\texttt{$\ell_0$ Norm}: we computed the mean of the non-zero activations of each ReLU Layer in our models when processing a set of input data. 
This metric is closely related to energy consumption and can be considered an alternative that does not rely on ASIC simulators. As a result, it can be applied to any architecture, offering broader applicability.

\subsection{Evaluation Metrics}
In order to qualitatively estimate the effectiveness of the
attack against the specific model’s grid set considered, we
introduce two novel distinct metrics: the \textit{Effectiveness Score Function} (ESF) and the \textit{Attack Success Rate} (ASR).
\par
% In order to qualitatively estimate the effectiveness of the attack against the specific \textcolor{red}{model's grids} \textcolor{blue}{set} considered, we introduce the \textit{Effectiveness Score Function} (ESF). 
The ESF goal is to understand the impact of MSHAA on the victim model when deployed. Therefore, with ESF we measure the MSHAA returned model $\tilde{h}_{\mathfrak{c}^*}$ and the legitimate $h_{\mathfrak{c}^*}$ based on the hijack metric $\mathcal{E}$.
Formally, ESF is defined as follows:
\begin{equation}
     \mathscr{S}(\mathfrak{C}) = \frac{
         \mathcal{E} ( \tilde{h}_{\mathfrak{c}^*}, \mathcal{S}^{Test} ) 
         - 
         \mathcal{E} ( h_{\mathfrak{c}^*}, \mathcal{S}^{Test} )
     }
     {
         \underset{\mathfrak{c} \in \mathfrak{C}}{\max} \{\mathcal{E}(h_{\mathfrak{c}}, \mathcal{S}^{Test})\} - 
         \mathcal{E} (    h_{\mathfrak{c}^*}, \mathcal{S}^{Test}    )
     }.
\end{equation}

ESF takes the difference between a chosen metric $\mathcal{E}$ of the models $\tilde{h}_{\mathfrak{c}^*}$ (see Equation~\ref{best_poison}) and $h_{\mathfrak{c}^*}$ (see Equation~\ref{best_val}) normalizing it with the difference between the maximum possible chosen metric of a model $h_\mathfrak{c}$ with $\mathfrak{c} \in \mathfrak{C}$, and again the chosen metric by $h_{\mathfrak{c}^*}$.\\
This function allows us to evaluate our attack with any metric $\mathcal{E}$, for the purpose of this study, with regards to the hijack metric considered:
\begin{itemize}
    \item \textit{Generalization Metric}. $\mathcal{E}$ is the loss function computed on the original validation set;
    \item \textit{Latency Metric}. $\mathcal{E}$ is the latency while processing the test set.
    \item \textit{Energy Consumption} or \textit{$\ell_0$ Norm}. $\mathcal{E}$ is the estimated energy consumed by the model while processing the test set. When testing the attack in the SpeechCommands case, as we could not compute the \texttt{Energy} metric, we evaluated the quality of the attack using the \texttt{$\ell_0$ Norm}, by adopting $\mathcal{E}$ to be the $\ell_0$ Norm.
\end{itemize}
This Effectiveness Score function allows us to give a normalized score that sums up the effectiveness of the MSHAA, as a matter of fact:
\begin{itemize}
    \item \textit{Successful}, when $ESF > 0$, the MS phase to return a model with higher $\mathcal{E}$ compared to $h_{\mathfrak{c}^*}$. If the score is equal to $1.0$, then the returned model $\tilde{h}_{\mathfrak{c}^*}$ is the one among the considered models to have the highest $\mathcal{E}$.
    \item \textit{Invariant}, when $ESF = 0.0$, the attack did not sway the MS phase, and the returned model is $\tilde{h}_{\mathfrak{c}^*} = h_{\mathfrak{c}^*}$, \textit{i.e.} the returned model is also the legitimate one. 
    \item \textit{Unsuccessful}, $ESF < 0.0$ imply that the attack made the MS phase return a model of less $\mathcal{E}$ compared to $h_{\mathfrak{c}^*}$.
\end{itemize}  
\par
We define the ASR as a simplification of the ESF. In particular, we define the ASR as a boolean variable of a successful or unsuccessful attack, and therefore the $ASR = 1$ if $ESF > 0$, $ASR = 0$ otherwise. 
With this metric, we are interested in understanding when an attack is successful in terms of increasing the hijack metric. 

% \section{Experimental Settings --- OLD}

% \subsection{Case Studies}
% We designed three distinct case studies to test the MSHAA attack performance: two yield from the Computer Vision (CV) field, and the remaining one from Speech Recognition (SR), all in the classification task. \\
% We opted to test two distinct application domains (CV and SR) to understand the generalization of the attack in different AI scenarios. These datasets were imported using the corresponding PyTorch libraries.

% \paragraph{MNIST (CV)~\cite{lecun2010mnist}} 
% It is a dataset of bilevel $28 \times 28$ handwritten digits divided into 10 classes: one for each digit from 0 to 9. 
% The victim models considered for this case are FeedForward Neural Networks, with hyperparameters grid concerning the number of neurons per layer and the number of layers themselves. 
% Our parameter grid consists of the following:
% \begin{itemize}
%     \item number of layers = $[1, 2, ..., 10]$;
%     \item number of neurons = $[32, 64, 128]$;
%     \item learning rate = $[0.0001, 0.0005, 0.001, 0.005, 0.01, 0.05]$.
% \end{itemize}
% Amounting to a total of 180 models: 30 for each learning rate.
%Regarding the specific hyperparameters, for the number of layers, we trained the network with layers 1 to 10 layers, with each layer having 32, 64, or 128 neurons. Then, these 30 models were trained using 6 different learning rates: 0.0001, 0.0005, 0.001, 0.005, 0.01, 0.05.\\
 %\textbf{ADD the excact grid}. 
% The HVAE comprises only fully connected layers and is trained using Binary Cross Entropy as a reconstruction loss ($\mathcal{L}_{\mathrm{rec}}$). 
% To train these HVAEs (for all the test cases considered), we considered different architectures and learning rates and then performed a model selection on these models. Ultimately for the attack, we used the one, among the ones trained, with the highest hijacking cost $Hj_{cost}$ (see Eq. \ref{cost}).  

% \paragraph{CIFAR10 (CV)~\cite{cifar10}} 
% It is a dataset of colored $32 \times 32$ images of various subjects belonging to 10 classes: airplane, automobile, bird, cat, deer, dog, frog, horse, ship, and truck. 
% In this case study the victim models are DenseNets \cite{huang2017densely}, of which we adapted the implementation done by \cite{PyTorchDenseNet}. The considered hyperparameters grid sees the number of dense blocks and the number of neurons for the fully connected layer which feeds the output one. Our parameter grid consists of the following:
% \begin{itemize}
%     \item number of dense blocs = $[2, 3, ..., 8]$;
%     \item fully-connected number of neurons = $[128, 256, 512]$;
%     \item learning rate = $[0.0001, 0.0005]$.
% \end{itemize}
% All in all, we trained 42 models for this case study.
%For the number of dense blocks, we had networks with 2, 3, 4, 5, 6, 7, and 8 blocks. Meanwhile for the number of neurons for the fully connected layer, we chose 128, 256, or 526. These 21 models were then trained using either 0.001 or 0.005 as learning rate.\\
%.\textbf{ADD the exact grid.}
% For CIFAR10, the HVAE adopted is composed of 2D convolutional layers, and the adopted reconstruction loss ($\mathcal{L}_{\mathrm{rec}}$) is the Mean Square Error.

% \paragraph{Speech Commands (SR)~\cite{speechcommandsdataset}} 
% It is a dataset composed of audio files of about 1 second long (around 16000 frames long) belonging to 35 classes of different commands spoken by different people. Here, the victim models are Convolutional Neural Networks composed of 1D convolutional layers, and the considered hyperparameters are the number of convolutional layers and the width of the fully connected layer that feeds the output one (code adapted from \cite{PyTorchSpeechCommands}).
% Our parameter grid consists of the following:
% \begin{itemize}
%     \item number of 1-dimensional convolutional layers = $[2, 4, 6, 8]$;
%     \item learning rate = $[0.01, 0.05]$.
% \end{itemize}
% Therefore, we trained 16 models for the classification of the SpeechCommands dataset.
% We chose to work using networks having 2, 4, 6, or 8 1-dimensional convolutional layers, and for the number of neurons for the fully connected layer, we chose either 128 or 256. These 8 models were then trained using either 0.001 or 0.005 as learning rate.\\
% For this Speech Recognition case study, the HVAE are made of 1D convolutional layers, with the Mean Square Error as the reconstruction loss ($\mathcal{L}_{\mathrm{rec}}$).

% \subsection{Hijack Metrics} % footnote does not work well due to balance in main.tex
% Regarding the hijack metrics considered, these were computed as follows:
%     \begin{itemize}
%         \item \texttt{Generalization Metric}. This hijack metric consists of the loss obtained by our models when processing the original, untampered validation set
%         \item \texttt{Latency Metric}. Obtained measuring the overall processing time of a given set of input data.
%         \item \texttt{Energy Consumption}. As stated before this estimation was computed by an ASIC simulator \footnote{\url{https://github.com/iliaishacked/sponge_examples}} \footnote{\url{https://github.com/Cinofix/sponge_poisoning_energy_latency_attack}} adapting the functions already developed for \cite{shumailov2021sponge} and \cite{cina2022energy}.\\
%         As this tool was not compatible with the specific architecture used for the classification models of the SpeechCommands dataset, this was the only case in which we did not consider this specific metric.
%         \item \texttt{$\ell_0$ Norm}. To obtain this metric we computed the mean of the non-zero activations of each ReLU Layer in our models when processing a set of input data.
%     \end{itemize}


==> tables/attack-evaluation-BB-complete.tex <==
\begin{tabularx}{0.45 \textwidth}{>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X |>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X}
\toprule
 & \texttt{Gener.} & \texttt{Latency} & \texttt{Energy} & \texttt{$\ell_0$} \\
\midrule
MNIST & 100.00\% & 100.00\% & 100.00\% & 100.00\% \\
CIFAR10 & 100.00\% & 100.00\% & 100.00\% & 100.00\% \\
SpeechC. & 100.00\% & 0.00\% & N/A & 0.00\% \\
\bottomrule
\end{tabularx}

==> tables/attack-evaluation-BB-lr-neuron.tex <==
\begin{tabularx}{0.45 \textwidth}{>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X |>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X}
\toprule
 & \texttt{Gener.} & \texttt{Latency} & \texttt{Energy} & \texttt{$\ell_0$} \\
\midrule
MNIST & 100.00\% & 83.33\% & 100.00\% & 100.00\% \\
CIFAR10 & 83.33\% & 50.00\% & 33.33\% & 50.00\% \\
SpeechC. & 100.00\% & 50.00\% & N/A & 50.00\% \\
\bottomrule
\end{tabularx}

==> tables/attack-evaluation-BB-lr.tex <==
\begin{tabularx}{0.45 \textwidth}{>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X |>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X}
\toprule
 & \texttt{Gener.} & \texttt{Latency} & \texttt{Energy} & \texttt{$\ell_0$} \\
\midrule
MNIST & 100.00\% & 100.00\% & 66.67\% & 83.33\% \\
CIFAR10 & 100.00\% & 50.00\% & 50.00\% & 100.00\% \\
SpeechC. & 100.00\% & 50.00\% & N/A & 0.00\% \\
\bottomrule
\end{tabularx}

==> tables/attack-evaluation-WB-complete.tex <==
\begin{tabularx}{0.45 \textwidth}{>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X |>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X}
\toprule
 & \texttt{Gener.} & \texttt{Latency} & \texttt{Energy} & \texttt{$\ell_0$} \\
\midrule
MNIST & 100.00\% & 100.00\% & 100.00\% & 100.00\% \\
CIFAR10 & 100.00\% & 0.00\% & 100.00\% & 100.00\% \\
SpeechC. & 100.00\% & 0.00\% & N/A & 0.00\% \\
\bottomrule
\end{tabularx}

==> tables/attack-evaluation-WB-lr-neuron.tex <==
\begin{tabularx}{0.45 \textwidth}{>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X |>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X}
\toprule
 & \texttt{Gener.} & \texttt{Latency} & \texttt{Energy} & \texttt{$\ell_0$} \\
\midrule
MNIST & 100.00\% & 94.44\% & 100.00\% & 100.00\% \\
CIFAR10 & 100.00\% & 33.33\% & 50.00\% & 50.00\% \\
SpeechC. & 100.00\% & 50.00\% & N/A & 0.00\% \\
\bottomrule
\end{tabularx}

==> tables/attack-evaluation-WB-lr.tex <==
\begin{tabularx}{0.45 \textwidth}{>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X |>{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X | >{\raggedleft\arraybackslash}X}
\toprule
 & \texttt{Gener.} & \texttt{Latency} & \texttt{Energy} & \texttt{$\ell_0$} \\
\midrule
MNIST & 100.00\% & 100.00\% & 66.67\% & 83.33\% \\
CIFAR10 & 100.00\% & 100.00\% & 100.00\% & 100.00\% \\
SpeechC. & 100.00\% & 50.00\% & N/A & 0.00\% \\
\bottomrule
\end{tabularx}
